Infinite-state games with finitary conditions

We study two-player zero-sum games over infinite-state graphs with boundedness conditions. Our first contribution is about the strategy complexity, i.e the memory required for winning strategies: we prove that over general infinite-state graphs, memoryless strategies are sufficient for finitary B\"uchi games, and finite-memory suffices for finitary parity games. We then study pushdown boundedness games, with two contributions. First we prove a collapse result for pushdown omega B games, implying the decidability of solving these games. Second we consider pushdown games with finitary parity along with stack boundedness conditions, and show that solving these games is EXPTIME-complete.

==> winning_regions.tex <==
\subsection{Characterizations of the winning regions}

We revisit the constructions used in Section~3 to describe the winning regions
for finitary B\"uchi objectives, in order to describe them using modal mu-calculus formulae.

The winning region for bounded uniform B\"uchi objectives was obtained in Proposition~\ref{prop:mem_bounded_uniform_buchi}
as a fixpoint computation, which can be expressed by the following modal mu-calculus formula:
$$\nu Y, \Attreve_B\left( F \cap \Pre(Y) \right)\ ,$$
or equivalently, using the $B$-approximant:
$$\nu Y \cdot \mu_B X,\ \left( F \cap \Pre(Y) \right)\ \cup \ \Pre(X)$$
Following Proposition~\ref{prop:mem_uniform_buchi}, the winning region for uniform B\"uchi objectives was obtained
as a fixpoint:
$$\mu Z \cdot \nu Y, \Attreve_B\left( (F \cup Z) \cap \Pre(Y) \right)\ .$$
However, the last step to define the winning region for bounded B\"uchi objectives 
involves an infinite union, see Proposition~\ref{prop:mem_fin_buchi}.
We can \textit{informally} express it by:
$$\mu T \cdot \left(\bigcup_{B \in \N} \mu Z \cdot \nu Y, \Attreve_B((F \cup Z \cup T) \cap \Pre(Y))\right)\ .$$

In order to be able to compute the winning region, we prove
that this infinite union collapses, \textit{i.e}:
$$\bigcup_{B \in \N} \WE(\uni\bucfb) = \WE(\uni\buc(F,N))\ ,$$
for some $N$. 
Note that this implies a collapse of the two outmost greatest fixpoints; the winning region is then computed by:
$$\mu T \cdot \nu Y, \Attreve_N((F \cup T) \cap \Pre(Y))\ .$$

If the bound $N$ is computable, then the formula above can be made into a modal mu-calculus formula,
and evaluated over the pushdown arena.
